VGF: Value-Guided Fuzzing -- Fuzzing Hardware as Hardware

As the complexity of logic designs increase, new avenues for testing digital hardware becomes necessary. Fuzz Testing (fuzzing) has recently received attention as a potential candidate for input vector generation on hardware designs. Using this technique, a fuzzer is used to generate an input to a logic design. Using a simulation engine, the logic design is given the generated stimulus and some metric of feedback is given to the fuzzer to aid in the input mutation. However, much like software fuzzing, hardware fuzzing uses code coverage as a metric to find new possible fuzzing paths. Unfortunately, as we show in this work, this coverage metric falls short of generic on some hardware designs where designers have taken a more direct approach at expressing a particular microarchitecture, or implementation, of the desired hardware. With this work, we introduce a new coverage metric which employs not code coverage, but state coverage internal to a design. By observing changes in signals within the logic circuit under testing, we are able to explore the state space of the design and provide feedback to a fuzzer engine for input generation. Our approach, Value-Guided Fuzzing (VGF), provides a generic metric of coverage which can be applied to any design regardless of its implementation. In this paper, we introduce our state-based VGF metric as well as a sample implementation which can be used with any VPI, DPI, VHPI, or FLI compliant simulator, making it completely HDL agnostic. We demonstrate the generality of VGF and show how our sample implementation is capable of finding bugs considerably faster than previous approaches.

==> background/afl/afl.tex <==
\Tuba{This section could be shortened..}
American Fuzzy Lop (AFL) is a mutational fuzzer which employs instrumentation in the
target program to generate a control-flow based coverage map. AFL can be
thought of as a dynamic analysis framework which discovers edges in a
control-flow graph by providing inputs to the application being tested.
Errors in the application are detected by recording when the application
crashes, the input given to the application, and a core dump containing the
backtrace, memory mappings, and status of global and local variables.


% When launching an application, the AFL driver maps a \SI{64}{\kibi\byte} area
% of memory as System-V shared memory and zeroes its contents. It then creates
% the environment variable \lstinline[style=ccode]{__AFM_SHM_ID} storing the ID
% of the shared memory. AFL then performs a two part primitive check in the 
% target application for instrumentation. The first part of the check is to
% ensure that the ASCII sequence \lstinline[style=ccode]{__AFL_SHM_ID} is present
% in the binary. This is done using the \lstinline[style=ccode]{strstr()}
% function over the binary image. How this string is used by the target
% application is not explicitly checked. The second part of the check is by
% performing a \emph{dry run}, where no inputs are given to the application.
% After the dry run, AFL checks the shared memory area for changes. If its
% content was modified, AFL assumes the application to be instrumented.

% \begin{lstlisting}[style=ccode,caption={Example AFL instrumentation. Each basic
% block is assigned a unique number or label which is used to identify the
% position in code.  Control-flow paths are identified by combining two labels
% together.},
% label={lst:afl_instrumentation}]
% /* code */
% if(<condition>) {
% 	current_location = <COMPILER_GENERATED_NUMBER_0>;
% 	shared_memory[current_location ^ previous_location]++;
% 	previous_location = current_location >> 1;
% 	/* code */
% } else {
% 	current_location = <COMPILER_GENERATED_NUMBER_1>;
% 	shared_memory[current_location ^ previous_location]++;
% 	previous_location = current_location >> 1;
% 	/* code */
% }
% /* code */
% \end{lstlisting}

% The instrumentation used by AFL on target applications is summarized in Listing
% \ref{lst:afl_instrumentation}. AFL labels every basic block with a unique
% identifier. It then uses a combination of the current basic block's label
% and the previous basic block's label to index into the hash map. The value at
% that particular index is incremented by one. New paths in execution are
% discovered by analyzing which indices in the hash map have been incremented.
% AFL sets the previous location to the current location's label shifted down by
% one as to avoid issues with tight loops. That is, in a loop containing only one
% basic block as its body allowing
% \lstinline[style=ccode]{previous_location = current_location}
% results in
% \lstinline[style=ccode]{0 == current_location ^ previous_location}
% thus always indexing at location 0 in the hash map.

% To improve performance, AFL implements a \emph{fork server}, which is embedded
% as part of the instrumentation. The purpose behind the fork server is to
% avoid expensive calls to \lstinline[style=ccode]{execve()} when spawning a new
% instance of the process to be fuzzed. Instead, when the process is first
% started and it reaches the \lstinline[style=ccode]{main()} function, it
% communicates with the AFL driver. Inter-process communication between the fork
% server and AFL is done through standard POSIX pipes on file descriptors 198 and
% 199 for AFL-to-process and process-to-AFL, respectively. When AFL issues a go,
% the fuzzed process invoques the \lstinline[style=ccode]{clone()} system call
% through the use of the POSIX \lstinline[style=ccode]{fork()} function. The
% parent process sends the PID of the child to AFL, and performs a
% \lstinline[style=ccode]{waitpid()} on the child. Data modified in the child
% process is handled by the kernel through copy-on-write semantics, severely
% reducing overhead. When the child process finishes execution, the fork server
% reaps it and communicates the exit status back to AFL and waits to be commanded
% for the next round of execution. AFL can then examine the hash map for
% control-flow information and mutate the input accordingly.


==> background/verilator/verilator.tex <==
% \Tuba{This section could be shortened..}
% \Xiaolong{Mainly shortended the limitation section.}


% As a simulator, Verilator\cite{snyder2013verilator} uses an intermediate C/C++ representation to build the emulation process, and this section discusses the generation of the intermediate C++ representation code.

% \subsubsection{Working Procedure of Verilator}

% After initialization and preprocessing, lexical analysis with Flex~\cite{flex} is performed in the Verilator process, and then parsing is made with Bison~\cite{Bison}. 
% The compilation process produces an abstract semantic tree (AST) representation of the design, identified in Verilator as an ASTNetlist type.
% Verilator iteratively traverses the AST to refine, optimize, and construct the internal design model. 
% % The AST units are first linked in the process. In addition, function variables are linked to their definitions.
% %The AST units are linked in the process, while function variables are linked to their definitions. \Xiaolong{What're the AST units, function variable and linked?}
% Specifically, Verilator divides each module in the hardware design source code into sequential and combinatorial designs, builds separate functions, and connects the function containing the hardware design to the top-level simulation function.
% After that, it performs further optimizations, including code coverage, assertions, X-elimination, inline function insertion, and dead code removal.

% % The design is then pseudo-flattened with additional modifications and optimizations, mainly for module references, function inlining, loop unrolling, variable lifetime analysis, lookup table generation, always splitting, and logic gate simplification.
% % \Xiaolong{What's the meaning of pseudo-flattened?}
% % Verilator then reorders the code to ensure that ``always'' statements run from top to bottom with no loops.

% % Verilator eliminates much of the flattening of the model so that the same module may be called and used in multiple places. They localize variables, merge similar functions, extend macros to the C primitives, and propagate constants.
% % At this point, Verilator's internal design model is completed and code generation on the C++ model design can proceed.\Xiaolong{What's the meaning of this sentence?}
% Nevertheless, the difference between a hardware design that runs in parallel and a software design that runs in serial (regardless of multithreading) is still a difference in operation.
% Verilator deconvolves the time-sequence logic for hardware emulation and reorganizes the "always" statement to ensure serial execution.
% % {\color{blue} @Weimin: please write this section. Thank you. }

% \orlando{There is also an issue with verilator's handling of possible logic states. Verilator only supports 1 and 0 as logic states, but the SystemVerilog standard mandates also X, U, Z, strong high, and strong low values. Incorrect treatment of these logic values can result in incorrect fuzzing results, as proper fidelity of the design under testing is not being properly simulated.}\Xiaolong{This point is put in 2.3.3.}

% % How conversion works at a high level.
% \subsubsection{C++ Code Conversion}
% Regarding the C++ code conversion, Verilator acquires the original design's AST through a SystemVerilog compiler. Then, despite various optimization stages, Verilator completes a mapping of a Verilog AST to a C++ AST. At the end of the process, Verilator generates C++ code in a pattern similar to code generation in software compilation. Verilator generates hardware-independent C++ code for the simulation driver in this procedure.
% %% Verilator acquires the original design's AST through a SystemVerilog compiler. Despite various optimization stages,  Verilator completes a mapping of a Verilog AST to a C++ AST, and at the end of the process, Verilator generates C++ code in a pattern similar to code generation in software compilation. In this procedure, Verilator additionally generates hardware-independent C++ code for the simulation driver.
% % Testbench driver model as C++ code.
% Verilator constructs the C++ design by exporting the inline, symbol table and constant pool within this sequence. In the model's subsequent output, the simulator's peripheral design code is written to the file first, followed by the model's C++ code. The peripheral design code is partially prewritten in \texttt{V3EmitCMain.cpp} and partially created during runtime by \texttt{V3EmitCModel.cpp}.

% %\medskip
% %\noindent\textbf{Limitations of Verilator:} 
% \subsubsection{Limitations of Verilator}
% Despite its sophistication, Verilator has several limitations which we expand upon below.
% % \Tuba{These limitations could be summarized using the current bullet points without the detailed explanations and those explanations could be placed in the Appendix.. }
% % \Xiaolong{Done with Bold.}

% \noindent\textbf{Inability to model multiple clock domains:} There is no real running clock in Verilator -- the clock signal trigger is the time when the \texttt{eval()} function is called. As a result, Verilator cannot simulate asynchronous (clockless) logic. When using multiple clocks simultaneously, the different intervals of the clock triggers are not simulated, and the triggers of multiple clocks are treated as \texttt{eval()} with the same characteristics.

% \noindent\textbf{Inaccuracy in translation:} In converting Verilog to C++, Verilator performs additional optimization techniques, such as the insertion of inline functions and loop unrolling. However, Verilator only ensures the equivalency between Verilog designs and C++ programs at the behavioral level. Thus, Verilator cannot assess the prospective behavior of design which targets a particular FPGA or ASIC and cannot manage potential problems caused by a particular logic gate design \orlando{check grammar}.

% \noindent\textbf{Ignoring portions of the SystemVerilog standard:} Verilator is not compliant with the complete IEEE 1364 (Verilog) and IEEE 1800 (SystemVerilog) standards and assumes that the target design allows it to optimize synchronous logic. Moreover, Verilator does not accept most non-synthetic code and cannot model \texttt{high-impedance} and \texttt{don't care}. In the end, as a cycle-based simulator, Verilator cannot be used for timing simulation, back-annotated netlists, asynchronous (unclocked) logic, and timing operations, such as disallowing \# statements.


\subsection{The Workflow of Verilator}
\label{app:hdl_conversion}
In the field of hardware emulation, Verilator is a widely adopted simulator that employs an intermediate C/C++ representation for constructing the emulation process\cite{snyder2013verilator}. The ensuing discussion focuses on generating this intermediate C++ representation code.

Verilator's process starts with initialization and preprocessing, followed by lexical analysis using Flex~\cite{flex} and parsing with Bison~\cite{Bison}. The outcome of the compilation process is an abstract semantic tree (AST) representation of the design, identified as an ASTNetlist type in Verilator. To refine, optimize, and construct the internal design model, Verilator iteratively traverses the AST.

Specifically, Verilator segregates each module in the hardware design source code into sequential and combinatorial designs, builds separate functions, and connects the function containing the hardware design to the top-level simulation function. Subsequent optimizations include code coverage, assertions, X-elimination, inline function insertion, and dead code removal.

A significant difference exists between hardware designs that operate in parallel and software designs that run in serial, even when multithreading is employed. Verilator untangles the time-sequence logic for hardware emulation and reorganizes the "always" statement to ensure serial execution.
\subsubsection{C++ Code Conversion}
During the C++ code conversion, Verilator acquires the original design's AST through a SystemVerilog compiler. Verilator maps a Verilog AST to a C++ AST despite various optimization stages. The final step entails generating C++ code in a pattern akin to code generation in software compilation. Verilator generates hardware-independent C++ code for the simulation driver in this procedure.

Verilator constructs the C++ design by exporting the inline, symbol table, and constant pool within this sequence. The simulator's peripheral design code is written to the file first, followed by the model's C++ code in the subsequent output. The peripheral design code is partially prewritten in \texttt{V3EmitCMain.cpp} and partially created during runtime by \texttt{V3EmitCModel.cpp}.

\subsubsection{Limitations of Verilator}
Despite its sophistication, Verilator exhibits several limitations:

\noindent\textbf{Inability to model multiple clock domains:} Verilator lacks a real running clock, as the clock signal trigger is the moment when the \texttt{eval()} function is called. Consequently, Verilator cannot simulate asynchronous (clockless) logic. When employing multiple clocks concurrently, the different intervals of the clock triggers are not simulated, and the triggers of multiple clocks are treated as \texttt{eval()} with identical characteristics.

\noindent\textbf{Inaccuracy in translation:} Verilator employs additional optimization techniques during Verilog-to-C++ conversions, such as inline function insertion and loop unrolling. However, Verilator only guarantees equivalency between Verilog designs and C++ programs at the behavioral level. Therefore, Verilator cannot evaluate the prospective behavior of a design targeting a specific FPGA or ASIC and cannot address potential issues arising from a particular logic gate design.

\noindent\textbf{Ignoring portions of the SystemVerilog standard:} Verilator does not fully comply with the complete IEEE 1364 (Verilog) and IEEE 1800 (SystemVerilog) standards, assuming that the target design permits the optimization of synchronous logic. Verilator does not support most non-synthetic code and cannot model \texttt{high-impedance} and \texttt{do not care} states. As a cycle-based simulator, Verilator is unsuitable for timing simulation, back-annotated netlists, asynchronous (unclocked) logic, and timing operations, such as disallowing \# statements.

Verilator is a powerful hardware emulation tool that relies on an intermediate C++ representation to build the emulation process. However, it is essential to be aware of its limitations, including its Inability to model multiple clock domains, potential inaccuracies in translation, and non-compliance with portions of the SystemVerilog standard. Despite these drawbacks, Verilator remains a widely used and valuable tool in hardware emulation, providing an efficient means of generating C++ code for hardware designs.

%% \begin{itemize}
	%% \item An inability to model multiple clock domains.
	
	%% In Verilator, there is no real running clock, and the clock signal trigger is actually the time when the eval() function is called. As a result, Verilator cannot simulate asynchronous (clockless) logic. Verilator, on the other hand, can handle synchronous digital logic circuits with one or more clocks that can be connected together in the same time domain during model generation inside Verilator. When using multiple clocks simultaneously, the different intervals of the clock triggers are not simulated, and the triggers of multiple clocks are treated as eval() with the same characteristics.
 
	%% \item Inaccuracy in Translation
	
	%% In the process of converting Verilog to C++, Verilator performs additional optimization techniques, such as the insertion of inline functions and loop unrolling. However, Verilator ensures that Verilog and C++ designs output identical signals and results. Despite the loss of implementation specifics of the hardware's behavior, it may be inferred that this translation is behaviorally equivalent. Since equivalency is at the behavioral level, it is impossible for Verilator to assess the prospective behavior of a program executing on a particular FPGA or ASIC, and it is unable to manage potential problems caused by a particular logic gate design.
	
%     \item Combinational loops
	
% 	Similar to the time domain in sequential logic, the sensitivity domain for combinational logic is presented in the combinational logic graph model.%{\color{green}(If anyone require additional information, I can organize the contents of V3Order.cpp lines 542 to 605)}
 
	%% \item Ignoring portions of the SystemVerilog standard.
	
    %% \begin{itemize}
        %% \item Verilator is not compliant with the complete IEEE 1364 (Verilog) and IEEE 1800 (SystemVerilog) standards and assumes that the target design allows it to optimize synchronous logic.
        %% \item Since Verilator is cycle-based, it cannot be used for timing simulation, back-annotated netlists, asynchronous (unclocked) logic, or in general any signal changes involving the concept of time, such as disallowing \# statements (which are usually required to model Phase-Locked Loops).
        %% \item Verilator does not accept most non-synthetic code, except for things like \$ display(), \$ finish(), \$ fatal(), part \$ assert, etc.
        %% \item The verilator is two-valued logic instead of four-valued logic (not modeling for high-impedance and don't care).

    %% \end{itemize}	
	%\item Something else?
%% \end{itemize}

%% For the remainder of this work, we assume that limitations on Verilator are engineering issues that can be solved with some time and effort. We assume that Verilator's generation of a C++ model is both compliant to the SystemVerilog HDL standard and is as accurate as possible.


==> img/fsm_all.tex <==
\begin{subfigure}[c]{0.475\columnwidth}
    \centering
    \begin{tikzpicture}[
    		node distance=1.5cm,
    		auto,
    		every state/.style={
    			thick,
    			circle,
    			color=blue!75,
    			fill=blue!15,
    			minimum size=0.75cm,
    			inner sep=0cm,
    			font=\footnotesize\ttfamily
    		},
    		bend angle=15,
    		-latex',
    	]
    	
        \node[state, initial left] (s0) {};
        \node[state, below right of=s0] (s1) {};
        \node[state, below left of=s1] (s2) {};
        \node[state, above left of=s2, accepting] (s3) {};
        
        \path   (s0) edge[bend left] node[font=\ttfamily\footnotesize] {1} (s1)
                (s1) edge[bend left] node[font=\ttfamily\footnotesize] {1} (s2)
                (s2) edge[bend left] node[font=\ttfamily\footnotesize] {1} (s3)
                (s0) edge[loop right] node[font=\ttfamily\footnotesize] {0} (s0)
                (s1) edge[loop right] node[font=\ttfamily\footnotesize] {0} (s1)
                (s2) edge[loop above] node[font=\ttfamily\footnotesize] {0} (s2)
            ;
    \end{tikzpicture}
    \caption{State transition diagram for the finite state machine.}
\end{subfigure}%
\hfill%
\begin{subfigure}[c]{0.475\columnwidth}
    \centering
    \begin{tikzpicture}[
    		node distance=1.5cm,
    		auto,
    		every state/.style={
    			thick,
    			circle,
    			color=blue!75,
    			fill=blue!15,
    			minimum size=0.75cm,
    			inner sep=0cm,
    			font=\footnotesize\ttfamily
    		},
    		bend angle=15,
    		-latex',
    	]
    
    \node[state, initial left] (s0) {};

    \path (s0) edge[loop right] (s0);
    
    \end{tikzpicture}
    \caption{Control-flow graph for simulation loop with microcode implementation. Only one node remains.}
\end{subfigure}
\begin{comment}
\begin{subfigure}{\columnwidth}
    \centering
    \begin{tikzpicture}[
    		node distance=2cm,
    		auto,
    		every state/.style={
    			thick,
    			circle,
    			color=blue!75,
    			fill=blue!15,
    			minimum size=1.0cm,
    			inner sep=0cm,
    			font=\footnotesize\ttfamily
    		},
    		bend angle=15,
    		-latex',
    	]
        
        \node[state, initial left] (s0) {};
        \node[state, below left of=s0] (s1) {};
        \node[state, below of=s0] (s2) {};
        \node[state, below right of=s0] (s3) {};
        
        \path   (s0) edge[loop above] (s0)
                (s0) edge[bend right] node[anchor=east,text width=1.5cm, align=right, font=\ttfamily] {0/0xaa} (s1)
                (s1) edge[bend right] (s0)
                (s0) edge[bend right] node[font=\ttfamily] {1/0xbb} (s2)
                (s0) edge[bend left] node[font=\ttfamily] {2/0xcc} (s3)
                (s2) edge[bend right] (s0)
                %(s3) edge[bend left] (s0)
            ;
    \end{tikzpicture}
    \caption{Control-flow graph for simulation loop with conditional statements. Basic blocks match that of state changes.}
\end{subfigure}\\
\end{comment}

==> prevlimits/prevlimits.tex <==
\begin{comment}

\subsection{Reexamining C++ conversion}
\Tuba{Don't we discuss this in Section 1.1 An Illustrative Example? I think this section is redundant...}\dean{Agreed.}
We start by examining the high-level SystemVerilog description of a Finite State Machine (FSM) as provided in Listing \ref{lst:high_level}. The next state computation is constructed with a combination of \lstinline[style=vcode]{case} and \lstinline[style=vcode]{if} statements. When transforming this construct to an equivalent C++ model using Verilator, the code shown in Listing \ref{lst:verilator_descriptive} is obtained. Explicit control-flow information is inferred using the ternary operator \lstinline[style=ccode]{?:} in C++. When built, this code is readily instrumented by AFL in a way where edges in the control-flow graph are readily discoverable. As new edges are discovered during the fuzzing process, the mutational engine in AFL can be guided to generate better inputs to map coverage in the core. This translates to AFL being capable of moving the state machine forward in a more concise way.

%Descriptive SystemVerilog HDL FSM on Listing \ref{lst:verilator_descriptive}. Explicit control-flow information can be obtained. Interestingly, this is only available in the implementation of the output function. The transition function utilizes a table lookup mechanism to set the next state. AFL-based instrumentation yields possible execution paths, however, as the output function can still be instrumented. \textbf{Find out why this happens. Is it because we are using an enum? What happens if we use localparam or constants instead?}

\begin{lstlisting}[style=ccode,caption={Fragment of Verilator-generated code for a descriptive FSM design.},label={lst:verilator_descriptive}]
    // ...
    vlSelf->d_out = (1U & ((0U == 
            (IData)(vlSelf->fsm__DOT__state))
        ? (IData)(vlSelf->d_in)
        : ((1U == (IData)(vlSelf->fsm__DOT__state))
            ? (~ (IData)(vlSelf->d_in))
            : ((2U == (IData)(vlSelf->fsm__DOT__state))
                & (IData)(vlSelf->d_in)))));
    __Vtableidx1 = (((IData)(vlSelf->d_in) << 2U)
        | (IData)(vlSelf->fsm__DOT__state));
    vlSelf->fsm__DOT__next_state =
        Vfsm__ConstPool__TABLE_h8ec40a36_0[__Vtableidx1];
    // ...
\end{lstlisting}

We perform the same analysis on the same FSM under a microarchitecture-specific as outlined in Listing \ref{lst:fsm_asic}. Relevant portions of the converted C++ code are shown on Listing \ref{lst:verilator_ucode}. Verilator populates an array which it uses to construct the microcode ROM table, then utilizes the array to assign to the next state computation. There is no explicit control-flow information in the way the next state computation is generated. The ternary operator is used once, but it is meant to set the initial state of the register. Because there is no explicit control-flow information, AFL's instrumentation is incapable of obtaining any coverage information on how to move the state machine forward.

% Microcoded FSM example translated into C++ uses bitshifts and lookups into an array on Listing \ref{lst:verilator_ucode}. No explicit control-flow information can be obtained. AFL-based instrumentation yields no paths.

\begin{lstlisting}[style=ccode,caption={Fragment of Verilator generated code for microcoded FSM design.},label={lst:verilator_ucode}]
    // ...
    vlSelf->fsm__DOT__ucode_rom[0U] = 0U;
    vlSelf->fsm__DOT__ucode_rom[1U] = 3U;
    vlSelf->fsm__DOT__ucode_rom[2U] = 5U;
    // ...
    vlSelf->fsm__DOT__state = ((IData)(vlSelf->res)
    			? 0U : (3U & (vlSelf->fsm__DOT__ucode_rom
    				[(((IData)(vlSelf->fsm__DOT__state)
    						<< 1U)
    					| (IData)(vlSelf->d_in))]
    				>> 1U)));
    // ...
\end{lstlisting}

We must then conclude that the choice of implementation affects the generated code. Moreover, the generated code may not be readily instrumentable by AFL to be able to detect changes in hardware state. Therefore, this methodology is not applicable to all designs.

\end{comment}

==> swhw/swhw.tex <==
\begin{comment}
%%%% DISCUSSION MADE IRRELEVANT

\subsection{Application Specific HDL Styles}

\begin{figure*}
    \centering
    \caption{Fuzzing workflow and instrumentation.}
    \label{fig:hdl_workflow}
\end{figure*}

We start our discussion with the way HDL is written and the standard HDL workflow. The style utilized in writing HDL depends on the final target. The overall workflow is described in Figure \ref{fig:hdl_workflow}. After a design description is written and tested, it is converted into a lower level representation which allows for other tools to map it to a domain-specific target. These domain-specific targets present variations in the way the HDL is written.

\subsubsection{Descriptive HDL}
We can find very descriptive HDL styles, which employ the most high-level constructs. We show an example of this style in Listing \ref{lst:high_level} where a portion of the HDL describes a finite state machine. Code written in this style give the most freedom to the synthesis tool to generate the underlying hardware. Unfortunately, this freedom comes at the cost of the designer losing control over the logic being generated. Synthesis tools will attempt to optimize designs done this way over its preset constraints. However, it becomes difficult to constrain the synthesis tool to generate a particular type of hardware primitive.

\begin{lstlisting}[style=vcode,caption={A finite state machine description in high level SystemVerilog HDL.},label={lst:high_level}]
module fsm(input clk, res, d_in, output d_out);
    typedef enum bit[1:0] {
            STATE_A, STATE_B, STATE_C
        } state_list;
    state_list state, next_state;
    always_comb @(*) begin
        next_state = state;
        case(state)
            STATE_A: if(d_in) next_state = STATE_B;
            STATE_B: if(~d_in) next_state = STATE_C;
            STATE_C: if(d_in) next_state = STATE_A;
            default: next_state = state;
        endcase;
    end
    /* ... */
endmodule
\end{lstlisting}

\end{comment}

\begin{comment}
%%%% MOVED TO INTRODUCTION and reworded there    


\subsubsection{HDL Targeting Technology Libraries}
\Tuba{I am not sure if this point serves our purpose as we use hardware simulation in our analysis and if I understand correctly, this paragraph talks about variations that could happen 
due to the synthesizing the hw for a target..Are we trying to say fuzzing RTL would be more 
comprehensize of the various behaviors than fuzzing at gate-level netlist level?}
\orlando{Precisely so, yes. One limitation of Verilator, and many open-source simulators for that matter, is that sometimes you need to emulate primitives that are technology library specific. As an example, if you are targeting a 7 Series FPGA from AMD/Xilinx you may end up using a hardware feature specific to that FPGA. If you want to do a simulation of that design, you need a way to emulate that hardware feature. This is something that commercial simulators such as Design Compiler or QuestaSIM have that the open-source tools do not have.}


\end{comment}

\begin{comment}
\begin{lstlisting}[style=vcode,caption={A finite state machine written in application-specific SystemVerilog HDL.},label={lst:fsm_asic}]
module fsm (input clk, res, d_in, output d_out);
    typedef struct packed {
            logic [1:0] next_state;
            logic       out;
        } ucode_line;
    typedef ucode_line ucode_table [0:7];
    logic [1:0] state;
    ucode_table ucode_rom = '{
            '{ next_state: 2'b00, out: 1'b0 },  /* 000 */
            '{ next_state: 2'b01, out: 1'b1 },  /* 001 */
            '{ next_state: 2'b10, out: 1'b1 },  /* 010 */
            '{ next_state: 2'b01, out: 1'b0 },  /* 011 */
            /* ... */
        };
    always @(posedge clk)
        if(res) state <= 2'b00;
        else state <= ucode_rom[{state, d_in}].next_state;
    assign d_out = ucode_rom[{state, d_in}].out;
endmodule
\end{lstlisting}
\end{comment}




% The event loop operations.

